Approximate analysis of biological systems by hybrid switching jump diffusion

In this paper we consider large state space continuous time Markov chains (MCs) arising in the field of systems biology. For density dependent families of MCs that represent the interaction of large groups of identical objects, Kurtz has proposed two kinds of approximations. One is based on ordinary differential equations, while the other uses a diffusion process. The computational cost of the deterministic approximation is significantly lower, but the diffusion approximation retains stochasticity and is able to reproduce relevant random features like variance, bimodality, and tail behavior. In a recent paper, for particular stochastic Petri net models, we proposed a jump diffusion approximation that aims at being applicable beyond the limits of Kurtz's diffusion approximation, namely when the process reaches the boundary with non-negligible probability. Other limitations of the diffusion approximation in its original form are that it can provide inaccurate results when the number of objects in some groups is often or constantly low and that it can be applied only to pure density dependent Markov chains. In order to overcome these drawbacks, in this paper we propose to apply the jump-diffusion approximation only to those components of the model that are in density dependent form and are associated with high population levels. The remaining components are treated as discrete quantities. The resulting process is a hybrid switching jump diffusion. We show that the stochastic differential equations that characterize this process can be derived automatically both from the description of the original Markov chains or starting from a higher level description language, like stochastic Petri nets. The proposed approach is illustrated on three models: one modeling the so called crazy clock reaction, one describing viral infection kinetics and the last considering transcription regulation.

==> discu.tex <==
\comMB{
Secondo le specifiche del giornale  "Discussion" deve:
This should explore the significance of the results of the work, not repeat them. A combined Results and Discussion section is often appropriate. Avoid extensive citations and discussion of published literature.
\\
}


==> tmp_simulation.tex <==
For what concerns our simulation algorithm it is similar to hybrid stochastic simulation methods based on dynamic partitioning (e.g. [1,2]).
In particular,  the main difference with respect to [1,2] is the heuristic defining the dynamic partitioning of the systems reactions in fluid and  discrete ones. Indeed, in our approach a reaction is defined discrete if at least one of its input and output quantities has reached its upper or lower bound (that are explicitly given as part of the model itself, see sec.3.2 for more details) 
N.B. Nel testo in sec.3.2 non diciamo cosi' ma assumiamo una partizione statica che forse potrebbe essere fuorviante, possiamo discuterne??
The advantage of considering the upper and lower bounds, instead of only the lower one as suggested in [1,2], could provide a better approximation when we consider a process  which can reach its boundaries with non-negligible probability.
For instance if we consider the simple system defined by the following four reactions:

\begin{eqnarray}
\notag
1A&\stackrel{k_1}{\rightarrow}& 100B\\
\notag
100B&\stackrel{k_2}{\rightarrow}&1A\\
\notag
B	&\stackrel{k_3}{\rightarrow}&C \\
\notag
C&\stackrel{k_4}{\rightarrow}& B\\
\end{eqnarray}
with $A_0,C_0 = 0$ and $B=1999$.

Then, we can observe that $A$ can reach its upper bound without having $B$ in its lower bound. In this situation our approach will always consider $k_1$ as  a discrete reaction; while the other approaches will consider it as a fluid reaction.
Obviously this is not a limitation of the approaches proposed in [1,2] which could be easily adapted to cope with this aspect.


[1]M. Griffith, T Courtney, J. Peccound, W.H. Sander. Dynamic partitioning for hybrid simulation of bistable HIV-1 transactivation network. Bioinformatic 2006; 22(22):2782-2789.
[2]H. Salis, V. Sotiropoulos and Y. N. Kaznessis. Multiscale Hy3S: Hybrid stochastic simulation for supercomputers. BMC Bioinformatics 2006;7:93.
